RAG based Question-Answering for Contextual Response Prediction System

Large Language Models (LLMs) have shown versatility in various Natural Language Processing (NLP) tasks, including their potential as effective question-answering systems. However, to provide precise and relevant information in response to specific customer queries in industry settings, LLMs require access to a comprehensive knowledge base to avoid hallucinations. Retrieval Augmented Generation (RAG) emerges as a promising technique to address this challenge. Yet, developing an accurate question-answering framework for real-world applications using RAG entails several challenges: 1) data availability issues, 2) evaluating the quality of generated content, and 3) the costly nature of human evaluation. In this paper, we introduce an end-to-end framework that employs LLMs with RAG capabilities for industry use cases. Given a customer query, the proposed system retrieves relevant knowledge documents and leverages them, along with previous chat history, to generate response suggestions for customer service agents in the contact centers of a major retail company. Through comprehensive automated and human evaluations, we show that this solution outperforms the current BERT-based algorithms in accuracy and relevance. Our findings suggest that RAG-based LLMs can be an excellent support to human customer service representatives by lightening their workload.

==> rag_best_setup_table.tex <==
\begin{table}[h]
\centering
\footnotesize
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Embedding} & \multicolumn{1}{l}{\textbf{Embedding size}} & \multicolumn{1}{l}{\textbf{R@1}} & \multicolumn{1}{l}{\textbf{R@3}} & \multicolumn{1}{l}{\textbf{R@5}} \\ \midrule
\textbf{USE}       & 512                                         & -                                & -                                & -                                \\
\textbf{SBERT}     & 768                                         & +15.36                           & +9.42                            & +8.22                            \\
\textbf{Vertex AI} & 768                                         & +21.55                           & +13.87                           & +11.85                           \\ \bottomrule
\end{tabular}
}

\caption{Performance of different embedding technique in the company data for ScaNN. Performance is shown as the (\%) of improvement wrt the lowest performing embedding (USE in this scenario)}
\label{tab_rag_best_combo}
\end{table}
